Cheetah: Optimizing and Accelerating Homomorphic Encryption for Private Inference

As the application of deep learning continues to grow, so does the amount of data used to make predictions. While traditionally, big-data deep learning was constrained by computing performance and off-chip memory bandwidth, a new constraint has emerged: privacy. One solution is homomorphic encryption (HE). Applying HE to the client-cloud model allows cloud services to perform inference directly on the client's encrypted data. While HE can meet privacy constraints, it introduces enormous computational challenges and remains impractically slow in current systems. This paper introduces Cheetah, a set of algorithmic and hardware optimizations for HE DNN inference to achieve plaintext DNN inference speeds. Cheetah proposes HE-parameter tuning optimization and operator scheduling optimizations, which together deliver 79x speedup over the state-of-the-art. However, this still falls short of plaintext inference speeds by almost four orders of magnitude. To bridge the remaining performance gap, Cheetah further proposes an accelerator architecture that, when combined with the algorithmic optimizations, approaches plaintext DNN inference speeds. We evaluate several common neural network models (e.g., ResNet50, VGG16, and AlexNet) and show that plaintext-level HE inference for each is feasible with a custom accelerator consuming 30W and 545mm^2.

==> 07-old_hardware_cs.tex <==


\section{ResNet-50 Case Study: Achieving Private Inferences at Plaintext Speed}
\label{sec:limits}

\subsection{Hot Kernel Design Space Exploration}

We conduct a design space exploration of each hot kernel required to implement HE operations 
to empirically estimate the speedup, power, and area gains.
For each kernel, we built a hardware accelerator using Catapult HLS 10.2 
and a commercially available 40nm technology library. % how did we model SRAM overheads
Functionality of each kernel implementation was verified against SEAL implementations.
Datapath and memory bitwidths were configured using HE parameters from HE-PTune.


To conduct the design space exploration, we swept hundreds of points per kernel.
Each design was configured with different memory bandwidth, datapath parallelism (i.e., hardware loop unrolling),
pipelining (i.e., initiation-interval), and clock frequency configurations.
We tabulate the power, performance, and area of these results using the Catapult RTL generation and power estimation flows.
We then use the results to identify three different Pareto optimal design points: power-performance, area-performance, and energy performance.

An example design space Pareto curve is shown in Figure{~\ref{fig:NTT_pareto}},
which shows the power-performance Pareto frontier for NTT.
We report the energy-optimal point from the power-performance Pareto frontiers for each kernel in Table{~\ref{tab:hls_ed2}}.
We use these Pareto optimal design points to inform our estimates of how much hardware acceleration benefits the overall speedup for HE.
Finally, we measure the speedups of the Pareto optimal points relative to SEAL software implementations on a Xeon server using the same HE parameters.


\begin{table}[t]
\begin{center}
\begin{small}
\caption{
Energy optimal accelerator implementations from the power-performance Pareto frontier.
}
\vspace{-.75em}
\label{tab:hls_ed2}
\begin{tabular}{c c c c c c}
\toprule
Kernel     & Latency & Power  & Area     & Energy & Speedup    \\
           &   (us)  &  (mW)  & (mm$^2$) &  (nJ)  & ($\times$) \\
\midrule
\headd     & 0.64    & 210    & 0.68     & 134    &  8.5       \\
\hemult    & 0.64    & 309    & 2.70     & 198    &  40        \\
\herotate  & 10.2    & 146    & 3.32     & 1500   &  8.7       \\
NTT        & 30.9    & 61.1   & 1.06     & 1890   &  1.16      \\
\bottomrule
\end{tabular}
\end{small}
\end{center}
\vspace{-2em}
\end{table}
%\hemult    & 0.33 & 630.1  & 2.72 & 207.9  \\
% PRNG     & 0.15 & 64.9   & 0.23 & 9.7    \\
% DiscGaus & 0.07 & 457.3  & 0.59 & 32.0   \\
% Enc      & 0.32 & 712.5  & 6.26 & 228.0  \\
% Dec      & 0.17 & 699.1  & 3.13 & 118.8  \\

\begin{figure}[t]
\centering
\includegraphics[width=\columnwidth]{figures/NTT_power.pdf}
\vspace{-1.75em}
\caption{DSE for NTT; Pareto frontier in red.}
\label{fig:NTT_pareto}
\vspace{-2em}
\end{figure}

\subsection{Using HE Acceleration to Achieve Plaintext Speeds}

We now demonstrate how combining HE-PTune and Sched-PA with hardware acceleration can achieve plaintext inference speeds by exploiting application and kernel parallelism.
Concretely, this manifests as intra-kernel and inter-kernel parallelism.
From the profiling results in Section{~\ref{sec:profiling}}, we estimated that HE is 3-4 orders of magnitude slower without acceleration.
To determine whether achieving this remaining speedup is possible, we use the Pareto optimal design points identified from our design space exploration to conduct a feasibility study of 
how much speedup custom hardware can achieve.
While it is well-known that deep learning contains abundant parallelism, the combined gains of hardware ASIC customization, HE-PTune, and Sched-PA are not.
Throughout this analysis, we will make pessimistic assumptions to ensure that we are providing a lower bound estimate.


\subsubsection{Intra-kernel speedups}

We first consider the benefit of exploiting parallelism and hardware acceleration for individual HE kernels.
The {\headd} and {\hemult} kernels provide substantial parallelism as the underlying computation consists of element-wise modular additions and multiplications which can be easily parallelized.
In the case of {\herotate~}and NTT, parts of the underlying computations occur sequentially while others can be parallelized such as the element-wise multiplications and butterfly computations.
Table{~\ref{tab:hls_ed2}} illustrates the speedups achievable by exploiting intra-kernel parallelism compared to SEAL library implementation on a 3GHz Intel SkyLake Xeon processor.
The results show that intra-kernel parallelism and acceleration only achieve limited speedup (around 10$\times$).
However, we note that these speedup results represent a lower bound as our baseline implementation is intentionally aggressive; 
HLS designs use a 40nm technology and operates at 1GHz while also taking a PPA penalty compared to full custom ASIC design of the Xeon core.

\begin{figure}[t]
\centering
\includegraphics[width=\columnwidth]{figures/ppa_total.pdf}
\vspace{-1em}
\caption{
Resources needed for plaintext speed using different optimization targets in 40nm and 5nm.
%based on ~\cite{TSMCscalingIEEE, tsmcnode28nm, tsmcnode20nm, tsmcnode16nm, tsmcnode5nm}.
%The last 3 groups are assuming scaling from 40nm to 5nm 
% following
}
\label{fig:total_cost}
\vspace{-1em}
\end{figure}

\begin{figure*}
\centering
\subfloat[Alexnet DSE]{\includegraphics[width=0.33\textwidth]{figures/alexnet_scatter.pdf}}
\subfloat[Time]{\includegraphics[width=0.33\textwidth]{figures/alexnet_stacked_pareto_latency.pdf}}
\subfloat[Energy]{\includegraphics[width=0.33\textwidth]{figures/alexnet_stacked_pareto_energy.pdf}}
\vspace{-0.5em}
\caption{
Units bug, but this is the idea.
Take away(s) should be:
(a) here's where resources are spent and things are compute bottle-necked.
(b) analyze pareto points to conclude if: PE parallelism, Lane parallelism, or kernel parallelism is best.}
\label{fig:acc_dse}
%\vspace{-2em}
\end{figure*}

\begin{figure*}
\centering
\subfloat[Alexnet Area breakdown]{\includegraphics[width=0.33\textwidth]{figures/alexnet_optimal_area_pie_chart.pdf}}
\subfloat[Time]{\includegraphics[width=0.33\textwidth]{figures/alexnet_stacked_pareto_latency.pdf}}
\subfloat[Energy]{\includegraphics[width=0.33\textwidth]{figures/alexnet_stacked_pareto_energy.pdf}}
\vspace{-0.5em}
\caption{
Now run everything on best point and show results.}
\label{fig:acc_dse}
%\vspace{-2em}
\end{figure*}

\subsubsection{Inter-kernel speedup}


Fortunately, neural networks contain abundant application-level parallelism which allows individual kernel invocations to operate in an embarrassingly parallel fashion (Figure~\ref{fig:cnn_example}).
For a length-N dot product, N partial products can be obtained in parallel by invoking \hemult~and \herotate~to the input image.
Only the following add reduction imposes some limitations on parallelism on dot products. 
More generally, if a layer contains a large number of input and output channels, convolutions across channels can be aggressively parallelized depending on the size of the model.


For example, consider CNN Layer6 in ResNet-50 ($f_w=3$, $w=64$, $c_i=c_o=64$). 
If each ciphertext contains a single input channel ($n=4096$), then all partial products can be computed with 36,864 \hemult~and \herotate~parallel kernel invocations.
The partial products for these layers cannot be parallelized since \hemult~must be performed before \herotate~in partial-aligned scheduling.
In \herotate~, domain conversion from evaluation to coefficient using INTT must be done before polynomial decomposition, but the remaining NTT to convert the domain of decomposed polynomials can be parallelized.
As a result, the degree of parallelism that can be exploited to compute a CNN layer is still on the order of thousands for ResNet-50, which is sufficient to achieve plaintext performance levels.
Our combined speedup estimate assumes sufficient hardware to execute all 
parallelizable kernels simultaneously using an optimized, fixed interconnect as all computation is scheduled statically.
Since our design is dominated by SRAMs and does not require dynamic data routing, 
we expect very little interconnect power and area overhead, similar to~\cite{dadiannao}.


\subsubsection{End-to-end latency and hardware cost estimates}

We now combine the parallelism afforded by intra- and inter-kernel parallelism with Cheetah and our design space exploration results to determine whether plaintext speed HE inference is possible.
Using the power, performance, and area results from the design space exploration, we construct an analytical model to estimate the power, performance, and area of implementing a HE inference accelerator.
Our analytical model pessimistically assumes that the results of each kernel are stored in a dedicate SRAM between each kernel execution, and that kernel accelerators and SRAMs are not reused.
In addition, we pessimistically do not assume inter-kernel pipelining (designs already have intra-kernel pipelining) or buffer reuse.

To estimate feasibility of plaintext inference speeds, for each Pareto optimal design point and HE kernel $k$ from our design space exploration, we take the recorded latency of the HLS implementation $t_{k,hw}$ and C++ CPU run time $t_{k,cpu}$ to compute the speed up from inter-kernel acceleration $s_{k,inter}$.
We then take the estimated speedup required to achieve plaintext $s_{k,pt}$ (from Figure{~\ref{fig:profile}}) and compute $K_k = s_{k,pt}/s_{k,inter}$.
The ratio $K_k$ represents the inter-kernel parallelism or parallel kernel factor needed to achieve plaintext inference speeds for HE kernel $k$.

We verify that each layer in ResNet50 has sufficient inter-kernel parallelism to satisfy the needed parallel kernel factors.% TODO: this check never fails
We then instantiate an accelerator which contains $K_k$ instances of each kernel $k$ to estimate the full system power, area, and energy needs to achieve plaintext end-to-end ResNet-50 inference in HE.
Power, area, and energy are computed by analytically scaling the HLS implementation power, area, and energy by the necessary parallel kernel factors.


The results of this analysis are shown in the left side of  Figure{~\ref{fig:total_cost}} for three different optimization targets: power, area, and energy.
We find optimizing for power favors lower frequency designs with larger designs due to high-degrees of inter-kernel parallelism.
The area-optimized design only incur a small increase in power overhead (6.4\%) while reducing area by 3.85$\times$. 
The energy optimal design achieve a middle ground with a small difference in power (2.4\%) and requiring only 33.7\% more area compared to the area-optimal design.
The key result is that to achieve plaintext inference on a 40nm technology node for ResNet-50, we would require an estimated 790\,W and 8097mm$^2$ using the area-optimal design.

Architecturally, 
we find that NTT favors inter-kernel parallelism
whereas the HE primitives strike a balance between
intra- and inter-kernel parallelism.
The underlying HE computations are embarrassingly-parallel
and are able to scale efficiency and performance within the kernel.
While NTT is also highly-parallel and amenable to acceleration,
it has more inter-loop-iteration dependencies and 
more complex memory-bank access patterns (e.g., butterfly access pattern).
Therefore, since we need extreme levels of speedup, NTT benefits more from
scale-out parallelism than scale-up (see Table~\ref{tab:hls_ed2}).

\subsubsection{Technology scaling}

% 

Our design space exploration uses a 40nm technology to estimate power and area due to limited access to advanced nodes.
To show the benefits of technology scaling, 
we report power and area estimates for 5nm using foundry-reported scaling factors.
Specifically, we use 0.2$\times$ power and 0.22$\times$ area to scale from 40nm to 16nm,
based on~\cite{TSMCscalingIEEE, tsmcnode28nm, tsmcnode20nm, tsmcnode16nm}. 
From 16nm to 5nm, the power and area scaling factors are 0.32$\times$ and 0.17$\times$, using~\cite{tsmcnode5nm} and a recent paper about 5nm technology from foundry~\cite{geoffrey2019tsmc}.
Together, the power and area scaling factors (40nm to 5nm) are 0.056$\times$ and 0.038$\times$, respectively.
Using these factors, 
we conclude that the resulting end-to-end chip resources---308mm$^2$ at 44.3W for area-optimized (see the right side of Figure~\ref{fig:total_cost})---are
within the range of feasibility as they are comparable to GPU chips in competitive technologies.



\subsubsection{Comparison with plaintext GPU inference}

The previous results show that with Cheetah optimizations
and sufficient hardware, HE inference latency can be equivalent to plaintext on a CPU.
While a significant amount of machine learning runs on CPUs~\cite{Hazelwood2018},
GPUs are increasingly leveraged to improve performance.
Profiling ResNet-50 on an NVIDIA 1080-Ti GPU with batch of 256
takes 435ms, and it is assumed (pessimistic for HE) that a single inference 
can be processed in 1.7ms.

This makes a GPU 58.8$\times$ faster than a CPU.
Given the remaining parallel kernel calls, 
the performance is \textit{theoretically} achievable
but would require all parallel calls be simultaneously processed
in hardware.
Instead, additional research on architectures for HE is required for more
efficient solutions.

\ignore{
\begin{table}[t]
\begin{center}
\begin{small}
\caption{
Estimated energy optimal accelerator designs scaled to 7nm node for each of the four hot kernels.
}
\label{tab:hls_scaled}
\begin{tabular}{c c c c c}
\toprule
Kernel  & Latency & Power & Area     & Energy \\
        &   (us)  &  (mW) & (mm$^2$) &  (nJ)  \\
\midrule
\headd     & 0.21   & 16.78  & 0.05 & 3.52  \\
\hemult    & 0.11   & 50.41  & 0.19 & 5.54  \\
\herotate  & 3.40   & 11.70  & 0.23 & 39.77 \\
NTT        & 10.30  & 4.89   & 0.07 & 50.35 \\
% PRNG     & 0.15 & 64.9   & 0.23 & 9.7    \\
% DiscGaus & 0.07 & 457.3  & 0.59 & 32.0   \\
% Enc      & 0.32 & 712.5  & 6.26 & 228.0  \\
% Dec      & 0.17 & 699.1  & 3.13 & 118.8  \\
\bottomrule
\end{tabular}
\end{small}
\end{center}
\vspace{-1em}
\end{table}

}

